AlphaClean: Automatic Generation of Data Cleaning Pipelines

The analyst effort in data cleaning is gradually shifting away from the design of hand-written scripts to building and tuning complex pipelines of automated data cleaning libraries. Hyper-parameter tuning for data cleaning is very different than hyper-parameter tuning for machine learning since the pipeline components and objective functions have structure that tuning algorithms can exploit. This paper proposes a framework, called AlphaClean, that rethinks parameter tuning for data cleaning pipelines. AlphaClean provides users with a rich library to define data quality measures with weighted sums of SQL aggregate queries. AlphaClean applies generate-then-search framework where each pipelined cleaning operator contributes candidate transformations to a shared pool. Asynchronously, in separate threads, a search algorithm sequences them into cleaning pipelines that maximize the user-defined quality measures. This architecture allows AlphaClean to apply a number of optimizations including incremental evaluation of the quality measures and learning dynamic pruning rules to reduce the search space. Our experiments on real and synthetic benchmarks suggest that AlphaClean finds solutions of up-to 9x higher quality than naively applying state-of-the-art parameter tuning methods, is significantly more robust to straggling data cleaning methods and redundancy in the data cleaning library, and can incorporate state-of-the-art cleaning systems such as HoloClean as cleaning operators.

==> acks.tex <==
NSF 1527765, 1564049.
Jiannan




==> cleaner.tex <==
\section{Cleaner}
After the detector returns $C_{d}$, the cleaner applies one of three actions: (1) impute the cell with a sensible default (consistent null symbol, mean value, most frequent value), (2) remove the record from the training set, or (3) flag the record as ``unpredictable'' return a null prediction or the most frequent label. The challenge is that search space is exponential in the number of cells. To address this problem, we use the prediction accuracy oracle to prioritize errors that correlate strongly with model mispredictions. This often greatly reduces the search space to a handful of sub-populations of data. \reminder{Sk needs to implement. We apply x algorithm to efficiently decide a per-cell repair}. For each cell $c \in C_{d}$, the cleaner returns a corresponding edit $e$.

==> compiler.tex <==
\section{Execution Layer}
This section describes how to optimize the intermediate representation.
\begin{enumerate}
    \item Describe the API for how users specify this.
    \item Loop fusion on adjacent operations.
\end{enumerate}

==> library.tex <==






==> opts.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/distributed.pdf}
    \caption{In each iteration, each worker starts with a subset of the priority queue (boxes).  The driver sends a subset of data transformations from $\Sigma$ (circles) to generate candidate programs (box-circles).  A series of synchronization points identify the globally top $\gamma$ candidates and redistributes them across the workers.   \label{fig:algo}}
\end{figure}


\section{Optimizations}\label{s:opts}
This section describes two important optimizations that allows \sys to generate cleaning programs in comparable runtimes as specialized systems.

\subsection{Dynamically Learning Pruning Rules}\label{s:dynlearn}
Our original hypothesis is that data cleaning problems exhibit structure that can be leveraged to accelerate a generic tree-search algorithm.   The core idea is to develop search pruning rules to minimize the number of candidate programs to evaluate.  Rather than hand-write pruning heuristics {\it a priori}, which is challenging when the user is presented with a new dataset, this optimization leverages the problem structure to learn pruning rules during the search process.


\stitle{Motivation}
The search algorithms in  most automatic data cleaning frameworks are carefully tuned for a specific quality function or class of quality functions. For example, the chase used in functional dependency resolution does not make an edit to the table unless it enforces at least one tuple's FD relationship.    Similarly, in entity matching problems, one restricts the search to only matching tuples that are likely to be similar based on some similarity metric.
These can be viewed as search pre-conditions that exploit the structure of the cleaning problem to a more tractable search space.
Note that these are not static optimizations: knowing how to prune the search space requires identifying and modeling the structure of the underlying data errors and how they interact with the data transformations.


\stitle{Approach}
When \sys executes the search algorithm on each block of data, it generates a cleaning program that optimizes the quality metric for that block.  In many cases, the dataset can be partitioned into a large number of blocks that each serve as sources of training examples for a learned pruning model.  Each transformation in a block's  cleaning program $p_b$ can be labeled as a positive training example in $\Sigma_b^+$, while all other transformations serve as negative examples $\Sigma_b^- = \Sigma - \Sigma_b^+$.
As \sys processes more blocks, the union of these training sets can be sufficient to train a classifier to predict whether a given transformation will be included in the optimal program.  In our approach, the prediction model $M(T): \Sigma \mapsto \{0,1\}$ is over the data transformations and not the data; is this sense, \sys learns static pruning rules in a dynamic fashion.    


Internally, \sys uses a Logistic Regression classifier that is biased towards false positives (i.e., keeping a bad search branch) over false negatives (e.g., pruning a good branch). This is done by training the model and shifting the prediction threshold until there are no False Negatives. 


\stitle{Featurization}
To use this approach, we use featurizers to transform each data transformation $T$ into a $k$-dimensional feature vector: \textsf{feat}: $T\mapsto\mathbb{R}^k$.
For example, recall the \texttt{find\_replace(NYC, NY, city\_code)} transformation in~\Cref{ex1}.
The expert is free to encode potential signals as part of the transformation.  For instance, the edit distance between the two literal parameters (e.g., NYC, NY) and an indicator vector to specify the attrbitue (e.g., city\_code).  

Notice that many data transformation can be modeled as a predicate that specifies which records to clean, target attributes to clean, and replacement values for those attributes.  Thus, the featurized transformation potentially allows a model to learn which records, which attributes, and what replacement values, are highly to contribute to the final cleaning program.  For instance, \sys may learn that \texttt{find\_replace} only makes sense for \texttt{city\_name}.  Similarly, it may learn that the replacement string should be similar in edit distance to the source string, and subsequently learn the appropriate edit distance threshould.

\stitle{Faster Data Quality Refinement}
\ewu{I emphasize this assuming the experiment exists!!!}
One benefit of learning a pruning model for {\it data transformations} rather than relation instances is that it can potentially be reused or fine-tuned for new, but structurally similar, data cleaning problems.  For instance, when users iteratively refine the data quality measure, the problem is largely the same, and \sys can intialize the search with the previously learned model.  This has the potential to learn  {\it across data cleaning problems} rather than across blocks within a single problem.   \ewu{We evaluate the benefits of re-using models during iterative refinement in Section~\ref{XXX}.}


\stitle{Discussion} We believe this is one of the reasons why a simple best-first search strategy can be effective.  For the initial blocks, \sys searches without a learned pruning rule in order to gather evidence.  Over time, the classifier can identify systematic patterns that are unlikely to lead to the final cleaning program, and explore the rest of the space.  In fact, this incremental learning process can be viewed from an active learning perspective to further target the exploration towards programs that will best improve the classification model.  

\sys uses linear classifier and feature extractors because it can be trained quickly with few examples.   However, we speculate that across a sufficient number of cleaning problems that share common set of data transformations (say, within the same department), we may adapt a deep learning approach to automatically learn the features themselves.  










\subsection{Parallelization}\label{s:parallel}
Composing and evaluating $Q(p'(R))$ is the single most expensive operation in the search procedure.   We now discuss how we parallelize its evaluation in shared memory and distributed settings, and the challenges when combining it with materialization.

\stitle{Shared Memory} In a naive, shared-memory implementation, we execute all expansions for a given $p\in P$ in parallel.  We materialize $p(R)$ in memory, and evaluate the quality of each $p' = p\circ T\ |\ T \in \Sigma$ in parallel using a  thread pool.  Each thread drops a given $p'$ if its quality is lower than $\gamma\times$ the maximum quality from the previous \texttt{WHILE} iteration or the local thread.  At the end of the \texttt{WHILE} iteration, the threads synchronize to compute the highest quality, and flush the remaining candidates using the up-to-date quality value.  The output of each $p'(R)$ can be retained or discarded using any cache replacement policy.  Our implementation uses Ray~\cite{ray} to schedule and parallelize the tasks.

 













==> statement.tex <==
\section{Synthesis Problem}
In this section, we describe the basic notation and problems addressed in this paper.

\subsection{Basic Notation}

\vspace{0.5em} \noindent \textbf{Transformations and Libraries: }
Let $R$ be a relation over a set of attributes $A$, and let $\mathcal{R}$ denote the set of all possible relations over $A$.
A data transformation is an operator over $\mathcal{R}$: 
\[T: \mathcal{R} \mapsto  \mathcal{R}\]
A library $L$ is a set of transformations, equipped with a binary operator denoting composition $T_1 \circ T_2 := T_1(T_2(R))$.
$L$ is a finite generating set of a universe $\mathcal{U}$, or the monoid of all transformations that can be constructed from compositions from the library.
The description length of a transformation $T \in \mathcal{U}$ (denoted by $\|T\|$) is the minimum number of compositions of library elements to generate $T$. 
\emph{We assume that data transformations are deterministic, do not change the cardinality of the relation, and assume perfect provenance.}

\begin{example}
Consider the example table below. An example of a transformation is the find-and-replace operator over the \textsf{city\_name} column, that is, find all cells that match some literal \texttt{x} and replace that cell with \texttt{y}. There are 6 possible find-and-replace transformations: Fr('San Francisco', 'New York'), Fr('New York City', 'New York'), Fr('New York', 'San Francisco'), Fr('New York City', 'San Francisco') ,Fr('San Francisco', 'New York City'), Fr('San Francisco', 'New York City'), which defines a library. The universe is every transformation that can be created from a sequence of find-and-replace operations.
\end{example}

\begin{table}[ht!]
\centering
\label{my-label}
\begin{tabular}{|l|l|l|}
\hline
\rowcolor[HTML]{000000} 
& {\color[HTML]{FFFFFF} city\_name}            & {\color[HTML]{FFFFFF} city\_code}   \\ \hline
1 & San Francisco                                & SF                                  \\ \hline
2& {\color[HTML]{FE0000} \textbf{New York}}     & NY                                  \\ \hline
3 & New York City                                & NY \\
\hline
\end{tabular}
\end{table}

\vspace{0.5em} \noindent \textbf{Quality Functions: } A quality function $Q$ maps every tuple $r \in R$ to an $|A|$ dimensional vector $[0,1]^{|A|}$, a value exactly equal to zero implies the cell is clean and a value greater than 0 describes the degree of dirtiness. We denote the aggregate sum of all quality values as: \[ \bar{Q} = \sum_{r \in R} \sum_{a \in A} Q(r)[a]\]

\begin{example}
Consider the example table below. Let $C$ be the set of cells that violate $\textsf{city\_name} \rightarrow \textsf{city\_code}$ and $\textsf{city\_code} \rightarrow \textsf{city\_name}$.
An example of a quality function is a function that maps every cell $c \in C$ to 1 and 0 other wise.
\end{example}

\begin{table}[ht!]
\centering
\label{my-label}
\begin{tabular}{|l|l|l|}
\hline
\rowcolor[HTML]{000000} 
& {\color[HTML]{FFFFFF} city\_name}            & {\color[HTML]{FFFFFF} city\_code}   \\ \hline
1 & San Francisco                                & SF                                  \\ \hline
2& {\color[HTML]{FE0000} \textbf{New York}}     & {\color[HTML]{FE0000} \textbf{NY}}                                  \\ \hline
3 & {\color[HTML]{FE0000} \textbf{New York City}}                              & {\color[HTML]{FE0000} \textbf{NY}} \\
\hline
\end{tabular}
\end{table}


\begin{example}
The quality function can also model numerical data. 
Consider data is that mostly Gaussian except for a few outliers. We can score each value by the number of standard deviations from the mean normalized the maximum deviation.
\end{example}

\subsection{Problem Statement}
The first problem addressed in \sys is the synthesis problem.

\begin{problem}[SYNTH(Q,R,L)]
Given a quality function $Q$, a relation $R$, and a library $L$, find a transformation $u$ of description length at most $k$ composed from the library that optimizes the quality function.
\[
u^* = \min_{u \in \mathcal{U}} \bar{Q}( u(R) )
\]
\[
\text{subject to: } \|u\| = k
\]
\end{problem}

\vspace{0.25em} \noindent\textbf{Complexity: } The synthesis problem is extremely general, and it is not our intention to directly solve this problem in full generality.
In fact, we can show that it is APX-Hard--that is, unless P=NP there does not exist a polynomial time approximation scheme.
However, we find that this optimization problem is a good starting point and an analysis of the complexity illustrates a number of important structural features of the problem.

\begin{proposition}
\textsf{SYNTH(Q,R,L)} is \textsf{APX-Hard}
\end{proposition}
\begin{proof}[Sketch]
Let $R$ be a single-attribute relation of Booleans. Let $L$ be the set of all assignments to a single value.
Given a list of $N$ Boolean clauses over all the boolean variables, let $Q$ assign to each record one minus the fraction of clauses that evaluate to true. This formulation is equivalent to MAX-SAT and solution to the optimization problem.
\end{proof}


\vspace{0.25em} \noindent\textbf{Remarks: } This reduction gives us some insight into what makes this problem computationally hard, and why practical data cleaning problems may not have those features. \emph{(1)} Arbitrary constraint satisfaction problems are challenging because all variables can interact. While this is certainly the case for arbitrary quality functions, in many cases, data errors are localized. For example, replacing \texttt{San Francisc} with \texttt{San Francisco} has no effect on the records referring to \texttt{New York City}.  \emph{(2)} Arbitrary constraint satisfaction involves assignments to all variables. On the other hand, in data cleaning, hopefully the majority of records in a dataset are clean so there is a structure that can be exploited.
 \emph{(3)} Constraint satisfaction does not model context, each variable is simply a Boolean value. In data cleaning, we can pragmatically exploit similarity. Similar records should be cleaned in similar ways.  

\subsection{Solution Overview}
We exploit these insights to develop a solution framework. The meta-algorithm is a greedy best-first tree search that maintains a size-limited frontier (i.e., it only expands nodes that are within a factor $\gamma$ of the current best solution).
We additionally hash intermediate results to remove search branches that lead to identical results and merge branches that have non-conflicting transformations that both lead to improved quality.

The tree-search is applied to limited blocks of data--over which it is computationally feasible. The blocking rules inferred from the quality specification or provided by the user as hints.
This synthesizes a local sequence of transformations for a small amount of data.
As the system applies the search to more and more blocks of data it builds a machine learning model of which transformations are likely to be included in the program.
Consider the set of transformations in Example 1. One could potentially learn that the only select transformations are ones where the edit distance between the two string parameters is small--pruning all transformations that map San Francisco-like strings to New York-like strings.




==> synth.tex <==
\section{Search Overview}
\sys applies a tree search to search through compositions of conditional assignments in the enumerated plan-space.
We now provide an overview of this search algorithm and optimizations.




\subsection{Naive Search Procedures}
In principle, any tree search algorithm over $P$ would be correct.
However, the traversal order and expansion policy is important in this search problem.  We describe the algorithmic and practical reasons why two naive procedures---breadth-first search (BFS) and depth-first search (DFS)---exhibit poor search runtimes.

\stitle{BFS} This approach extends each program in the search frontier with every possible data transformation in $\Sigma$.  To extend a candidate program $l_c$ with $T \in \Sigma$, it evaluates $Q((T\circ l_c)(R))$.  Unfortunately, the frontier grows exponentially with each iteration.  Additionally, evaluating every new candidate program $T\circ l_c$ can be expensive if the input relation is large.   Although the cost can be reduced by materializing $l_c(R)$, it is not possible to materialize all candidate programs in the frontier for all but the most trivial cleaning problems.    It is desirable to use asearch procedure that bounds the size of the frontier and the materialization costs.


\stitle{DFS} Depth-first search only needs to materialize the intermediate results for a single program at a time, however it is highly inefficient since the vast majority of programs that it explores will have low quality scores.  


\subsection{Core Search Algorithm}
Best-first search expands the most promising nodes chosen according to a specified cost function.
We consider a greedy version of this algorithm, which removes nodes on the frontier that are more than $\gamma$ times worse than the current best solution (\Cref{alg:main}).
Making $\gamma$ smaller makes the algorithm asympotically consistent but uses more memory to store the frontier, whereas $\gamma=1$ is a pure greedy search with minimal memory requirements.  

The frontier is modeled as a priority queue $P$ where the priority is the quality of the candidate program, and is initialized with a NOOP program with quality $Q(R)$.  
The algorithm iteratively extends all programs in the queue with less than $k$ transformations; a program $p$ is extended by composing it with a transformation $T$ in $\Sigma$.  If the resulting program $p'$ is in the language $L$, then we add it to the queue.
Finally, let $\bar{p}$ be the highest quality program in the queue.  The algorithm removes all programs whose quality is $<\gamma\times Q(\bar{p}(R))$ from the frontier.  
This process repeats until the candidate programs cannot be improved, or all programs have $k$ transformations.

In a naive and slow implementation, the above algorithm computes $p$'s quality by fully running $p$ on the input relation before running $Q$ on the result, explores all possible data transformation sequences, and runs sequentially.  One of the benefits of its simple structure is that it is amenable to a rich set of optimizations to prune the search space, incrementally compute quality functions, and parallelize the search.  In fact, we find that many optimizations in existing specialized cleaning systems can be cast in terms of the following classes.



\btitle{Static Pruning Rules} are boolean functions that take a candidate program $p$ as input and decides whether it should be pruned. \sys currently models static rules as regular expressions over $\Sigma$.  Static rules are can be viewed as filters over $L$.
\[\textsf{static\_rule}(p) \mapsto \{0,1\}\]
For example, since the find-and-replace operations are idempotent, i.e., $T(T(R)) = T(R)$, we may want to only consider the set of all sequences with no neighboring repeated transformations. Similarly, we may also want to prune all search branches that make no effect (i.e., find-and-replace New York with New York).
These two regular expressions alone reduce the above example's language by $48\%$ (from 226981 to 120050).
Other rules, such as avoiding changes that undo previous changes $T^{-1}(T(R)) = R$, are similarly easy to add.


\btitle{Dynamic Pruning Rules} also have access to the input relation and quality function, and can make instance-specific pruning decisions.
\[\textsf{dyn\_rule}(p, Q, R) \mapsto \{0,1\}\]
For example, suppose  $Q$ is based on functional dependencies and is cell-separable, and we want to ensure that cell-level transformations made by a candidate program $p$ individually improve $Q$.  In this case, we find the cells $C$ that initially violate the functional dependencies and ensure that the cells transformed by $p$ are all in $C$.  Applying this optimization, in addition to the others in \sys, to the example reduces the search space by $143\times$ from 226,981 candidate programs to only 1582.  

Since it can be challenging to hand-write pruning rules, \Cref{s:dynlearn} describes a dynamic approach that uses simple machine learning models to automatically identify the characteristics of candidate programs to decide whether a particular search brach will be promising.  In essence, it generates and refines static pruning rules during the search process.  



\subsection{Block-wise Tuning}
A major cost is that independent errors in the relation must be cleaned sequentially in the search algorithm.  For instance, records 2, 3, and 4 in~\Cref{ex1} exhibit independent errors and a fix for a given record does not affect the other records.  Thus, if each record were cleaned in isolation, the search space would be $O(|\Sigma|)$.  Unfortunately, the entire relation requires a program of three transformation to fix the records, which increases the search space to $O(|\Sigma|^3)$.

The main insight in block-wise cleaning is that many errors are local to a small number of records.  In these cases, it is possible to partition $R$ into a set of blocks $B_1,\cdots,B_m$, execute the search algorithm over each block independently, and concatenate their programs to generate the final cleaning program.  This gather-scatter approach can exponentially reduce the search space for each block, and reduces the cost of evaluating super-linear quality functions that require e.g., computing a pair-wise similarity scores for the input relation.    For example, quality functions derived from functional dependencies can define blocks by examining the violating tuples linked through the dependency.  Similarly, users can define custom partitioning functions or learn them via e.g., clustering algorithms.  In our current implementation, we partition the input relation by cell or row if the quality function is cell or row separable.




\stitle{Parallel Program Evaluation} It is clear that the candidate programs can be evaluated and pruning in a parallel fashion across multiple cores and multiple machines, and is one of the major innovations in modern planning systems.  However, unlike classic planning problems where communications are small due to the compact size of each state, \sys's state size is determined by the relation instance, and can lead to prohibitively high communication costs and memory caching requirements.   Section~\ref{s:parallel} describes how we manage the trade-offs when parallelizing \sys in shared memory and distributed settings.

\stitle{Materialization} Since each candidate program $p' = p\circ T$ is the composition of a previous candidate program and a transformation, an obvious optimization is to materialize the output of $p(R)$ and incrementally compute $p'(R)$ as $T(p(R))$ over the materialized intermediate relation.  Although this works well in a single threaded setting, memory and communication challenges arise when combining materialization with parallelization (\Cref{s:parallel}).








==> synthesizer.tex <==
\section{Synthesizer}
Given a the list of edits and cells, the synthesizer generates a Python program that given future unlabeled dirty data in the same schema will predict the the label. \sys converts the proposed edits into a lambda without any import dependencies. This allows for the detection predicate to be efficiently evaluated on new data, as well as be serialized so it can on future data without having to be retrained.


==> usecase.tex <==
\section{An Illustrative Example}


In this case, we are lucky; the joint optimization converges to a reasonable solution given enough time.  However, as we scale to more complex and larger scale problems, avoiding local optima becomes a daunting challenge.  Interactions between methods may not simply be redundancies, and improperly tuned techniques might even reverse the changes made by previous steps.  We arrived at a simple architecture to address this issue by rethinking the parameter search process.  For a given parameter setting, every data cleaning method in the pipeline suggests \emph{candidate} repairs to a dataset.  These repairs are aggregated into a large set of possible transformations to apply Then, a meta-algorithm searches over sequential compositions of the set of generated candidates.  The size of the search space can be controlled by how many parameter settings are considered and how coarse- or fine-grained the repairs are.  This process allows the system to leverage partial repairs from the pipeline when beneficial and naturally avoid problems of redundancy.


More importantly, this generate-then-search process is specialized to the idiosyncrasies of data cleaning.  Data cleaning is fundamentally a form of constraint satisfaction---easy to verify but hard to satisfy.  So, candidate generation can be much more expensive than accuracy evaluation (e.g., for Denial Constraints).  Existing search algorithms implicitly pipeline these two steps; whereas, we decouple these two steps where candidate repairs can be generated in a separate thread and the search algorithm can proceed independently.


In data cleaning, there is a chicken-and-egg problem, where accuracy is defined in terms of recovering the true values of cells in a database, but knowing the true values in advance would defeat the purpose of cleaning.  In practice, we often use a proxy for accuracy such as the satisfaction of integrity constraints, how well it fits a statistical model, or accuracy on gold standard data.  Given one of these proxy accuracy metrics, is black-box hyperparameter tuning sufficient for applications in data cleaning optimization?



A parameter generator thread supplies assignments to each of the data cleaning methods in the library and yields candidate repairs as they are generated to a set.  A greedy tree-search algorithm runs in parallel by sequencing candidate repairs and computing the resulting accuracy measure.  \sys can also execute in a divide-and-conquer fashion by generating candidate parameters on different partitions of data.  It also provides utilities for leveraging information across partitions, by learns a prediction model to estimate the expected improvement of different transformation operators (e.g., some library components might be irrelevant).  


